Conditions for Estimation of Sensitivities of Voltage Magnitudes to Complex Power Injections

Voltage phase angle measurements are often unavailable from sensors in distribution networks and transmission network boundaries. Therefore, this paper addresses the conditions for estimating sensitivities of voltage magnitudes with respect to complex (active and reactive) electric power injections based on sensor measurements. These sensitivities represent submatrices of the inverse power flow Jacobian. We extend previous results to show that the sensitivities of a bus voltage magnitude with respect to active power injections are unique and different from those with respect to reactive power. The classical Newton-Raphson power flow model is used to derive a novel representation of bus voltage magnitudes as an underdetermined linear operator of the active and reactive power injections; parameterized by the bus power factors. Two conditions that ensure the existence of unique complex power injections given voltage magnitudes are established for this underdetermined linear system, thereby compressing the solution space. The first is a sufficient condition based on the bus power factors. The second is a necessary and sufficient condition based on the system eigenvalues. We use matrix completion theory to develop estimation methods for recovering sensitivity matrices with varying levels of sensor availability. Simulations verify the results and demonstrate engineering use of the proposed methods.

==> defs/tables/04-20-22/meshed-table.tex <==
\begin{table*}[ht]
        \renewcommand{\arraystretch}{1.45}
        \caption{Test of analytical results for meshed Matpower test feeders at default operating point}
        \label{table:invertibility_bound_meshed}
        %\vspace{-3mm}
        \begin{center}
        \begin{tabular}{|c||c||c||c||c||c||c||c|}
        \hline
          & \multicolumn{2}{c||}{\textbf{Assumption Valid?}} &  \multicolumn{4}{c||}{\textbf{Quantity}}  &  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Thm. Holds?}}}\\
        \cline{1-7}
        \textbf{Case } &  $\dpdth \succ 0$ %& $\frac{1}{2}(\dpdth + \dpdth^T) \succ 0$ 
        & $\mathbf{J}^{-1}$ Exists & $\alpha_{\text{max}}- \alpha_{\text{min}}$ & $k_{\text{max}}-k_{\text{min}}$ & $\norm{\mathbf{M}^{-1}}^{-1}_2 \big\lVert \dpdth \big\rVert_2^{-1}$ & $\|\mathbf{M}^{-1} \Delta \mathbf{K} \dpdth \|_2$ & \\
        \hline
        case5\setfootnotemark\label{first} & Yes & Yes&  0.0 & 0.0 & 0.448 & 0.0 & \textcolor{ForestGreen}{Yes}\\
        \hline
        % case6 & Yes & Yes&  0.0 & 0.0 & 0.1472 & 0.0 & \textcolor{ForestGreen}{Yes}\\
        % \hline
        case9 & Yes & Yes&  0.0563 & 0.194 & 0.471 & 0.280 & \textcolor{ForestGreen}{Yes}\\
        \hline
        case14 & Yes & Yes&  0.138 & 0.434 & 0.0915 & 0.474 & \textcolor{ForestGreen}{Yes}\\
        \hline
        case24 & Yes & Yes&  $1.65 \times 10^{-3}$ & $8.70\times 10^{-3}$ & $0.0317$ & 0.0230 & \textcolor{ForestGreen}{Yes}\\
        \hline
        case30 & Yes & Yes&  0.192 & 0.591 & 0.1472 & 1.335 & \textcolor{Sepia}{No}\\
        \hline
        \end{tabular}
        \afterpage{\footnotetext[\getrefnumber{first}]{Theorem \ref{thm1:suff_cond} holds for all case 5 variants provided by \texttt{PowerModels.jl} except for: 1.) \texttt{case5\_db}, as its Jacobian is singular, as well as 2.) \texttt{case5\_sw} and 3.) \texttt{case5\_tnep}, as they have a single PQ bus.}}
        \end{center}
    \end{table*}

==> defs/tables/04-20-22/radial-table.tex <==
\begin{table*}[htb]
        \renewcommand{\arraystretch}{1.45}
        \caption{Test of analytical results for radial Matpower test feeders at default operating point}
        \label{table:invertibility_bound_radial}
        %\vspace{-3mm}
        \begin{center}
        \begin{tabular}{|c||c||c||c||c||c||c||c|}
        \hline
          & \multicolumn{2}{c||}{\textbf{Assumption Valid?}} &  \multicolumn{4}{c||}{\textbf{Quantity}}  &  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Thm. Holds?}}}\\
        \cline{1-7}
        \textbf{Case } &  $\dpdth \succ 0$ %& $\frac{1}{2}(\dpdth + \dpdth^T) \succ 0$ 
        & $\mathbf{J}^{-1}$  Exists & $\alpha_{\text{max}}- \alpha_{\text{min}}$ & $k_{\text{max}}-k_{\text{min}}$ & $\norm{\mathbf{M}^{-1}}^{-1}_2 \big\lVert \dpdth \big\rVert_2^{-1}$ & $\|\mathbf{M}^{-1} \Delta \mathbf{K} \dpdth \|_2$ & \\
        \hline
        case2 & Yes & Yes&  0.0 & 0.0 & 0.403 & 0.0 & \textcolor{ForestGreen}{Yes}\\
        \hline
        case5\_tnep & Yes & Yes&  0.0 & 0.0 & 0.4553 & 0.0 & \textcolor{ForestGreen}{Yes}\\
        \hline
        frankenstein\_00 & Yes & Yes&  0.0 & 0.0 & 0.4714 & 0.0 & \textcolor{ForestGreen}{Yes}\\
        \hline
        case4\_dist & Yes & Yes&  0.0 & 0.0 & 0.1472 & 0.0 & \textcolor{ForestGreen}{Yes}\\
        \hline
        % case10ba & Yes & Yes & 0.34293 & 2.833 & 0.5001 & 6.21 & \textcolor{Sepia}{No}\\
        case10ba & Yes & Yes & 0.34293 & 2.833 & $6.596 \times 10^{-3}$ & 6.21 & \textcolor{Sepia}{No}\\
        \hline
        % case12da & Yes & Yes & 0.0929 & 0.250  & 0.5103 & 5.38 & \textcolor{Sepia}{No}\\
        case12da & Yes & Yes & 0.0929 & 0.250  & 0.01072 & 5.38 & \textcolor{Sepia}{No}\\
        \hline
        case15da & Yes & Yes & $7.141 \times 10^{-8}$ & $2.041 \times 10^{-7}$& 0.6299 & $1.74 \times 10^{-6}$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        % case15nbr  & Yes & Yes & $7.14 \times 10^{-8}$ & $2.05 \times 10^{-7}$ & 0.266 & $1.76 \times 10^{-6}$ & \textcolor{ForestGreen}{Yes}\\
        case15nbr  & Yes & Yes & $7.141 \times 10^{-8}$ & $2.041 \times 10^{-7}$ & 0.0156 & $1.76 \times 10^{-6}$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        case16am   & Yes & Yes & 0.248 & 0.767 & 0.198 & $0.993$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        case16ci  & Yes & Yes & 0.198 & 0.54 & 0.206 & $0.40$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        %case17me   & Yes & Yes & 0.319 & 0.967 & 0.0062 & $17.55$& \textcolor{Sepia}{No}\\
        case17me   & Yes & Yes & 0.248 & 0.767 & 0.01204 & $17.55$& \textcolor{Sepia}{No}\\
        \hline
        case18     & Yes & Yes & 0.0588 & 0.1533 & 0.00573 & $3.0485$& \textcolor{Sepia}{No}\\
        \hline
        % case18nbr & Yes & Yes &  $1.43\times 10^{-4}$  & $4.08 \times 10^{-4}$ & 0.262 & $6.2 \times 10^{-3}$ & \textcolor{ForestGreen}{Yes}\\
        case18nbr & Yes & Yes &  $1.43\times 10^{-4}$  & $4.08 \times 10^{-4}$ & 0.0115 & $6.2 \times 10^{-3}$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        % case22     & Yes & Yes &  $0.164$    &  $0.495$      & 0.387 & $6.39$& \textcolor{Sepia}{No}\\
        case22     & Yes & Yes &  $0.164$    &  $0.495$      & $7.182 \times 10^{-3}$ & $6.39$& \textcolor{Sepia}{No}\\
        \hline
        % case28da   & Yes & Yes &  $6.25 \times 10^{-6}$ & $1.79 \times 10^{-5}$ & 0.328 & $5.0 \times 10^{-4}$ & \textcolor{ForestGreen}{Yes}\\
        case28da   & Yes & Yes &  $6.25 \times 10^{-6}$ & $1.79 \times 10^{-5}$ & $2.157 \times 10^{-3}$ & $5.0 \times 10^{-4}$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        %case33bw   & Yes & Yes & $0.670$ & $2.833$ & 0.202 & $27.82$& \textcolor{Sepia}{No}\\
        case33bw   & Yes & Yes & $0.670$ & $2.833$ & $2.732 \times 10^{-3}$ & $27.82$& \textcolor{Sepia}{No}\\
        \hline
        % case33mg  & Yes & Yes & $0.670$  & $2.83$ & 0.160 & $28.024$& \textcolor{Sepia}{No}\\
        case33mg  & Yes & Yes & $0.670$  & $2.83$ & $2.50 \times 10^{-3}$ & $28.024$& \textcolor{Sepia}{No}\\
        \hline
        %case34sa  & Yes & Yes & $0.0534$  & $0.238$ & 0.221 & $0.573$ & \textcolor{ForestGreen}{Yes}\\
        case34sa  & Yes & Yes & $0.0534$  & $0.238$ & 0.0166 & $0.573$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        case38si   & Yes & Yes & $0.670$  & $2.833$ & 0.160 & $17.792$& \textcolor{Sepia}{No}\\
        \hline
        %        case51ga   & Yes & Yes & $0.251$  & $0.701$ & 0.209 & $15.484$& \textcolor{Sepia}{No}\\
        case51ga   & Yes & Yes & $0.251$  & $0.701$ & $1.105 \times 10^{-3}$ & $15.484$& \textcolor{Sepia}{No}\\
        \hline
        %case51he   & Yes & Yes & $0.251$  & $0.701$ & 0.259 & $1.720$& \textcolor{Sepia}{No}\\
        case51he   & Yes & Yes & $0.119$  & $0.321$ & 0.0112 & $1.720$& \textcolor{Sepia}{No}\\
        \hline
        case69     & Yes & Yes & $0.100$   & $0.263$ & $0.123 \times 10^{-3}$ & $0.518$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        case70da    & Yes & Yes & $0.194$   & $0.523$ & $2.879 \times 10^{-3}$ & $9.820$& \textcolor{Sepia}{No}\\
        \hline
        case74ds    & Yes & Yes & $0.161$   & $0.429$ & $0.344 \times 10^{-3}$ & $30.25$& \textcolor{Sepia}{No}\\
        \hline
        case85     & Yes & Yes & $1.25 \times 10^{-6}$ & $3.57 \times 10^{-6}$   & 0.0191 & $1.28 \times 10^{-5}$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        %case94pi    & Yes & Yes & $5.86 \times 10^{-3}$ & $16.7 \times 10^{-3}$ & 0.030 & $0.0870$ & \textcolor{ForestGreen}{Yes}\\
        case94pi    & Yes & Yes & $5.86 \times 10^{-3}$ & $16.7 \times 10^{-3}$ & $1.082\times 10^{-3}$  & $0.0864$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        % case118zh   & Yes & Yes & $0.445$   & $1.412$ & $0.056$ & $22.53$& \textcolor{Sepia}{No}\\
        case118zh   & Yes & Yes & $0.445$   & $1.412$ & $0.5064 \times 10^{-3}$ & $22.53$& \textcolor{Sepia}{No}\\
        \hline
        case136ma   & Yes & Yes & $0.0309$ &  $0.09137$ & $0.135 \times 10^{-3}$ & $0.158$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        case141   & Yes & Yes & $1.493 \times 10^{-5}$   & $3.92 \times 10^{-9}$ & $5.496 \times 10^{-6}$ & $5.48 \times 10^{-7}$ & \textcolor{ForestGreen}{Yes}\\
        % case141   & Yes & Yes & $1.493 \times 10^{-5}$   & $3.92 \times 10^{-9}$ & $5.64 \times 10^{-5}$ & $5.48 \times 10^{-7}$ & \textcolor{ForestGreen}{Yes}\\
        \hline
        
        % &  \\
        % \cline{2-10}
        % \textbf{Bound} &&  0.055 & 0.090 & 0.037 &  0.0004 & 0.027 & 0.021 & 0.012 & 0.0025\\ 
        % \hline
        \end{tabular}
        \end{center}
    \end{table*}
